Reconstructing Recognizable 3D Face Shapes based on 3D Morphable Models

Many recent works have reconstructed distinctive 3D face shapes by aggregating shape parameters of the same identity and separating those of different people based on parametric models (e.g., 3D morphable models (3DMMs)). However, despite the high accuracy in the face recognition task using these shape parameters, the visual discrimination of face shapes reconstructed from those parameters is unsatisfactory. The following research question has not been answered in previous works: Do discriminative shape parameters guarantee visual discrimination in represented 3D face shapes? This paper analyzes the relationship between shape parameters and reconstructed shape geometry and proposes a novel shape identity-aware regularization(SIR) loss for shape parameters, aiming at increasing discriminability in both the shape parameter and shape geometry domains. Moreover, to cope with the lack of training data containing both landmark and identity annotations, we propose a network structure and an associated training strategy to leverage mixed data containing either identity or landmark labels. We compare our method with existing methods in terms of the reconstruction error, visual distinguishability, and face recognition accuracy of the shape parameters. Experimental results show that our method outperforms the state-of-the-art methods.

==> 7_response_letter.tex <==
\section{Response letter}
\subsection{ACKNOWLEDGEMENT}
We highly appreciate editors and the reviewers for their insightful comments and criticism on our manuscript, which have helped us improve both the content and the presentation of our work. We have tried our best to revise the paper based on them. We first summarize the major changes made in the revised version, including additional experiments performed. We then provide a detailed response to each comment.
\subsection{Summary of major changes}
The major changes to this manuscript are as follows:
\begin{itemize}
    \item We introduced a new metric, SIR-score, to measure the recognizability of the face shapes in Section 4. We revised our claims on contributions accordingly in the introduction and conclusion section, and added user studies to evaluate the effectiveness of the SIR-sorce metric in Section 4.2. We also added a comparison with other method using the SIR-score metric in Table 7.
    \item We re-wrote the formula of the loss function in Section 3.4 and the caption of Figure 2. 
    \item We conducted a quantitative evaluation on the LFW dataset(section 4.4)
\end{itemize}

\subsection{Detailed Responses to Each Reviewer}
\textbf{************Reviewer 1**************}
    
\textbf{Q: It would be even better if the authors can release their code for training.}

A: We have released our code on GitHub, which was also mentioned in abstract.

\textbf{************Reviewer 2**************}

\textbf{Q1:The proposed solution is basically to force the shape parameter space to have different centers and force the shape parameters to be clustered based on identity… It is really difficult to tell which one is correct just looking at the phong rendered meshes.}

A: We admit that it is not easy to tell the correctness by directly looking at phong rendered meshes. To better measure it, we propose the new SIR-score metric, which can quantitatively describe the recognizability of the face reconstruction. We have conducted a user study which shows that if two faces have a smaller SIR, their identities are easier to be distinguished. 
%Additionally, it can replace face recognition metric, and become novel metric of recognizability of the face reconstruction.

\textbf{Q2: Figure 2 and the associate section that describes the overview of the pipeline is not very clear. }

A: We have improved our explanation as mentioned in the major changes.

\textbf{Q3: For Figures 9 and 10, the ground truth mesh was not added to the results. As it is, in many of the examples the 3D face that best matches the shape of the picture is not generated by this method/ For example, Figure 7 4th row, the 3DFR produces a much better shape visually despite having a huge error in the error map.}

A: The experiment in Figure 7 is to reveal the consistency of the reconstructed shape of the face image under different conditions. Although in the fourth row of Figure 7, the reconstruction result of D3FR seems to be closer to the face of the origin, the reconstruction result of D3FR in the fifth row is very different from the fourth row, which illustrates the failure of disentangling the expression and pose from the face shape. Thus, the quantitative results show our method outperforms others. We have performed quantitative test to validate our method and added that into our paper.


\textbf{Q4: Figure 5 - to me the best result is in the first column, w/o SIR. }
A: Figure 5 shows the ablation study results of SIR losses. We consider the results with SIR has more variance and can better capture identity feature on face shape, like eyehole.

\textbf{Q5: Figure 11 - it is really difficult to tell which one is correct just looking at the phong rendered meshes,}

A: We were following most previous work [TTHMM17, LZZ∗18, SBFB19] when comparing the face geometries using Phong rendered meshes. Our aforementioned user study will give a better validation on the reconstruction quality. 


\textbf{************Reviewer 3**************}

\textbf{Q1: Some of the training details are missing. }

A: We have added the learning rate, the batch size, and the type of the optimizer for training. We have released our code on GitHub.


\textbf{Q2: The description of the loss function part (Sec 3.4) is a bit confusing. For example, $L_{pix}$ in Eq. 9 and $L_{pixel}$ in Eq. 11 represent two different losses, but the subscripts are similar. Losses are also defined hierarchically, which makes it difficult to get an easy understanding of the whole picture. In addition, the loss defined in Eq. 8 is the same as in Eq. 21, which is duplicated. And the $L_{SIR}$ is not clearly illustrated in the equations. Does $L_{id}$  in Eq. 17 represent SIR loss? Overall, the loss function part needs a re-organization to be more clear.}

A: We have fixed all the above descriptions.


\textbf{Q3: The experiment part can be further improved. For example, to evaluate the reconstruction stability and distinguishability, some quantitative evaluation on a larger scale of test data should be conducted.}

A: We have conducted more tests to evaluate stability and distinguishability on Bosphorus dataset and LFW dataset. We reported the SIR metric on Bosphorus dataset to evaluate the stability and distinguishability. And we also calculated the ratio of RMSE between pairs of images with the same identity and between pairs with different identities in LFW dataset to evaluate the stability and distinguishability.


\textbf{Q4: It is unclear to me if using shape parameters for face recognition is a reasonable way, in that face texture should contain more information to distinguish different person.}


A: We admit that face texture contains identity information, which can influence recognizability. However, we focus on the geometric discrimination in this paper, and thus consider the texture of faces out of the scope of our paper. This can be useful in applications where high-quality textures are unavailable (such as low light), and ensures more accurate 3D reconstruction that retains recognizable geometric features. The user study mentioned in the answer to Q1 of Reviewer 2 have demonstrated whether the meshes are sufficiently discriminative regarding the identity information.

